Outlier Suppression: Pushing the Limit of Low-bit Transformer Language Models

Transformer architecture has become the fundamental element of the widespread natural language processing~(NLP) models. With the trends of large NLP models, the increasing memory and computation costs hinder their efficient deployment on resource-limited devices. Therefore, transformer quantization attracts wide research interest. Recent work recognizes that structured outliers are the critical bottleneck for quantization performance. However, their proposed methods increase the computation overhead and still leave the outliers there. To fundamentally address this problem, this paper delves into the inherent inducement and importance of the outliers. We discover that $\boldsymbol \gamma$ in LayerNorm (LN) acts as a sinful amplifier for the outliers, and the importance of outliers varies greatly where some outliers provided by a few tokens cover a large area but can be clipped sharply without negative impacts. Motivated by these findings, we propose an outlier suppression framework including two components: Gamma Migration and Token-Wise Clipping. The Gamma Migration migrates the outlier amplifier to subsequent modules in an equivalent transformation, contributing to a more quantization-friendly model without any extra burden. The Token-Wise Clipping takes advantage of the large variance of token range and designs a token-wise coarse-to-fine pipeline, obtaining a clipping range with minimal final quantization loss in an efficient way. This framework effectively suppresses the outliers and can be used in a plug-and-play mode. Extensive experiments prove that our framework surpasses the existing works and, for the first time, pushes the 6-bit post-training BERT quantization to the full-precision (FP) level. Our code is available at https://github.com/wimh966/outlier_suppression.

==> tables/rotate_output_quantizer_cosine.tex <==
\begin{table*}[pht]
\footnotesize
    \centering
    \begin{adjustbox}{width=\textheight,totalheight=\textwidth,angle=90}
    \begin{tabular}{llllllllllllllllll}
        \toprule
        \multicolumn{2}{c}{\bf BERT-SQuAD v1.1} & \multicolumn{2}{c}{\bf BERT-CoLA} & \multicolumn{2}{c}{\bf BERT-STS-B} &
        \multicolumn{2}{c}{\bf RoBERTa-MNLI} & \multicolumn{2}{c}{\bf RoBERTa-SST-2} & \multicolumn{2}{c}{\bf RoBERTa-RTE} &
        \multicolumn{2}{c}{\bf BART-QQP} & \multicolumn{2}{c}{\bf BART-QNLI} & \multicolumn{2}{c}{\bf BART-MRPC}\\
            \cmidrule (l{2pt}r{2pt}){1-2}   
            \cmidrule (l{2pt}r{2pt}){3-4} 
            \cmidrule (l{2pt}r{2pt}){5-6} 
            \cmidrule (l{2pt}r{2pt}){7-8}
            \cmidrule (l{2pt}r{2pt}){9-10}
            \cmidrule (l{2pt}r{2pt}){11-12}
            \cmidrule (l{2pt}r{2pt}){13-14}
            \cmidrule (l{2pt}r{2pt}){15-16}
            \cmidrule (l{2pt}r{2pt}){17-18} 
        % & similarity  (\%)  &  & similarity  (\%)  &  & similarity  (\%) &  & similarity  (\%) &  & similarity  (\%)\\
        output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%) & output & cosine  (\%)\\
        \midrule
            layer.9.GELU &82.67 &layer.9.GELU &92.44 &layer.8.GELU &87.83 & layer.7.GELU &93.91 &layer.3.GELU &91.29 &layer.7.GELU &91.94 & layer.0.GELU (Decoder) &93.95 &layer.0.GELU (Decoder) &93.08 &layer.0.GELU (Decoder) &93.20\\
            layer.1.GELU (Decoder) &96.42 &layer.2.GELU (Decoder) &95.45 &layer.1.GELU (Decoder) &95.76\\
            layer.2.GELU (Decoder) &97.44 &layer.1.GELU (Decoder) &95.98 &layer.2.GELU (Decoder) &96.03\\
            layer.4.Attn-LN (Encoder-Decoder) &98.65 &layer.4.GELU (Decoder) &97.77 &layer.3.GELU (Decoder) &97.70\\
            layer.2.Attn-LN (Encoder-Decoder) &98.92 &layer.3.GELU (Decoder) &97.79 &layer.4.GELU (Decoder) &97.84\\
            layer.4.GELU (Decoder) &98.97 &layer.4.Attn-LN (Encoder-Decoder) &98.06 &layer.4.Attn-LN (Encoder-Decoder) &98.09\\
            layer.1.Attn-LN (Encoder) &99.17 &layer.2.Attn-LN (Encoder-Decoder) &98.51 &layer.2.Attn-LN (Encoder-Decoder) &98.52\\
            layer.3.GELU (Decoder) &99.22 &layer.1.Attn-LN (Encoder-Decoder) &99.11 &layer.3.Attn-LN (Encoder-Decoder) &99.04\\
            layer.5.Attn-LN (Encoder) &99.24 &layer.3.Attn-LN (Encoder-Decoder) &99.11 &layer.5.Attn-LN (Encoder) &99.07\\
            layer.1.Attn-LN (Encoder-Decoder) &99.25 &layer.5.Attn-LN (Encoder) &99.13 &layer.1.Attn-LN (Encoder-Decoder) &99.09\\
            layer.3.Attn-LN (Encoder-Decoder) &99.25 &layer.4.Attn-LN (Encoder) &99.16 &layer.4.Attn-LN (Encoder) &99.16\\
            layer.4.Attn-LN (Encoder) &99.27 &layer.1.Attn-LN (Encoder) &99.22 &layer.3.Attn-LN (Encoder) &99.31\\
            layer.0.GELU (Encoder) &99.30 &layer.0.Attn-LN (Encoder) &99.24 &layer.0.Attn-LN (Encoder) &99.33\\
            layer.3.Attn-LN (Encoder) &99.36 &layer.3.Attn-LN (Encoder) &99.33 &layer.1.Attn-LN (Encoder) &99.34\\
            layer.0.Attn-LN (Encoder) &99.39 &layer.0.GELU (Encoder) &99.37 &layer.0.GELU (Encoder) &99.36\\
            layer.2.Attn-LN (Encoder) &99.47 &layer.2.Attn-LN (Encoder) &99.48 &layer.2.Attn-LN (Encoder) &99.52\\
            layer.2.GELU (Encoder) &99.61 &layer.2.GELU (Encoder) &99.55 &layer.2.GELU (Encoder) &99.56\\
            layer.0.Attn-LN (Encoder-Decoder) &99.63 &layer.5.GELU (Decoder) &99.60 &layer.5.GELU (Decoder) &99.61\\
            layer.3.GELU (Encoder) &99.68 &layer.3.GELU (Encoder) &99.62 &layer.0.Attn-LN (Encoder-Decoder) &99.64\\
            layer.3.Attn-LN (Decoder) &99.82 &layer.1.GELU (Encoder) &99.65 &layer.1.GELU (Encoder) &99.66\\
            layer.5.Attn-LN (Encoder-Decoder) &99.84 &layer.0.Attn-LN (Encoder-Decoder) &99.66 &layer.3.GELU (Encoder) &99.69\\
            layer.5.Attn-LN (Decoder) &99.85 &layer.3.Attn-LN (Decoder) &99.81 &layer.3.Attn-LN (Decoder) &99.79\\
            layer.5.GELU (Decoder) &99.87 &layer.5.Attn-LN (Decoder) &99.86 &layer.5.Attn-LN (Encoder-Decoder) &99.82\\
            layer.5.GELU (Encoder) &99.89 &layer.5.Attn-LN (Encoder-Decoder) &99.87 &layer.5.Attn-LN (Decoder) &99.87\\
            layer.3.FFN-LN (Decoder) &99.89 &layer.4.GELU (Encoder) &99.89 &layer.3.FFN-LN (Decoder) &99.89\\
            layer.1.Context (Decoder) &99.91 &layer.3.FFN-LN (Decoder) &99.90 &layer.4.GELU (Encoder) &99.90\\
            layer.1.Context (Decoder) &99.91 &layer.5.GELU (Encoder) &99.91 &layer.1.Attn-LN (Decoder) &99.91\\
            layer.2.Context (Decoder) &99.92 &layer.4.FFN-LN (Decoder) &99.91 &layer.2.Attn-LN (Decoder) &99.91\\
            layer.2.FFN-LN (Decoder) &99.92 &layer.4.Attn-LN (Decoder) &99.91 &layer.5.GELU (Encoder) &99.91\\
            layer.1.Attn-LN (Decoder) &99.92 &layer.2.Attn-LN (Decoder) &99.91 &layer.4.Attn-LN (Decoder) &99.91\\
            layer.2.Attn-LN (Decoder) &99.92 &layer.1.Attn-LN (Decoder) &99.91 &layer.4.FFN-LN (Decoder) &99.92\\
            layer.0.FFN-LN (Decoder) &99.92 &layer.0.FFN-LN (Decoder) &99.92 &layer.2.FFN-LN (Decoder) &99.93\\
        % \midrule
        %     \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The sorted cosine similarity of the output at each module on BART models. We show the 32 most problematic ones with lowest cosine similarity.}
    \label{tab_bart_output_quantizer_cosine}
\end{table*}

